CustomCrafter: Customized Video Generation with Preserving Motion and Concept Composition Abilities

Customized video generation aims to generate high-quality videos guided by text prompts and subject's reference images. However, since it is only trained on static images, the fine-tuning process of subject learning disrupts abilities of video diffusion models (VDMs) to combine concepts and generate motions. To restore these abilities, some methods use additional video similar to the prompt to fine-tune or guide the model. This requires frequent changes of guiding videos and even re-tuning of the model when generating different motions, which is very inconvenient for users. In this paper, we propose CustomCrafter, a novel framework that preserves the model's motion generation and conceptual combination abilities without additional video and fine-tuning to recovery. For preserving conceptual combination ability, we design a plug-and-play module to update few parameters in VDMs, enhancing the model's ability to capture the appearance details and the ability of concept combinations for new subjects. For motion generation, we observed that VDMs tend to restore the motion of video in the early stage of denoising, while focusing on the recovery of subject details in the later stage. Therefore, we propose Dynamic Weighted Video Sampling Strategy. Using the pluggability of our subject learning modules, we reduce the impact of this module on motion generation in the early stage of denoising, preserving the ability to generate motion of VDMs. In the later stage of denoising, we restore this module to repair the appearance details of the specified subject, thereby ensuring the fidelity of the subject's appearance. Experimental results show that our method has a significant improvement compared to previous methods. Code is available at https://github.com/WuTao-CS/CustomCrafter

==> sections/7_checklist.tex <==
\newpage
\section{Reproducibility Checklist}
\textbf{Question1:} Includes a conceptual outline and/or pseudocode description of AI methods introduced? \\
Answer: Yes. \\
\textbf{Question2:} Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results? \\
Answer: Yes. \\
\textbf{Question3:} Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper? \\
Answer: Yes. \\
\textbf{Question4:} Does this paper make theoretical contributions? \\
Answer: Yes. \\
\textbf{Question5:} All assumptions and restrictions are stated clearly and formally? \\
Answer: Yes. \\
\textbf{Question6:} All novel claims are stated formally (e.g., in theorem statements)? \\
Answer: Yes. \\
\textbf{Question7:} Proofs of all novel claims are included? \\
Answer: Yes. \\
\textbf{Question8:} Proof sketches or intuitions are given for complex and/or novel results? \\
Answer: Yes. \\
\textbf{Question9:} Appropriate citations to theoretical tools used are given? \\
Answer: Yes. \\
\textbf{Question10:} All theoretical claims are demonstrated empirically to hold? \\
Answer: Yes. \\
\textbf{Question11:} All experimental code used to eliminate or disprove claims is included? \\
Answer: Yes. \\
\textbf{Question12:} Does this paper rely on one or more datasets? \\
Answer: Yes. \\
\textbf{Question13:} A motivation is given for why the experiments are conducted on the selected datasets? \\
Answer: Yes. \\
\textbf{Question14:} All novel datasets introduced in this paper are included in a data appendix? \\
Answer: Yes. \\
\textbf{Question15:} All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes? \\
Answer: Yes. \\
\textbf{Question16:} All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations? \\
Answer: Yes. \\
\textbf{Question17:} All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available? \\
Answer: Yes. \\
\textbf{Question18:} All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing? \\
Answer: NA. \\
\textbf{Question19:} Does this paper include computational experiments? \\
Answer: Yes. \\
\textbf{Question20:} Any code required for pre-processing data is included in the appendix? \\
Answer: Yes. \\
\textbf{Question21:} All source code required for conducting and analyzing the experiments is included in a code appendix? \\
Answer: Yes. \\
\textbf{Question22:} All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes? \\
Answer: Yes. \\
\textbf{Question23:} All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from ? \\
Answer: Partial. \\
\textbf{Question24:} If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results? \\
Answer: NA. \\
\textbf{Question25:} This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks? \\
Answer: Yes. \\
\textbf{Question26:} This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics? \\
Answer: Yes. \\
\textbf{Question27:} This paper states the number of algorithm runs used to compute each reported result? \\
Answer: Yes. \\
\textbf{Question28:} Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information? \\
Answer: NA. \\
\textbf{Question29:} The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank)? \\
Answer: No. \\
\textbf{Question30:} This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments? \\
Answer: Yes. \\
\textbf{Question31:} This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting? \\
Answer: Partial. \\


==> tables/ablation_study.tex <==
\begin{table}[]
    \centering
    \resizebox{0.48\textwidth}{!}{
   \begin{tabular}{lcccc}
   \toprule
    Method        & CLIP-T $\uparrow$  & CLIP-I $\uparrow$  & DINO-I $\uparrow$  & T. Cons. $\uparrow$  \\ \midrule
    w/o DWVSS     & 0.294  & 0.790    & 0.631  & 0.993  \\
    CustomCrafter & 0.318  & 0.786    & 0.627 & 0.994  \\ \bottomrule
    \end{tabular}
    }
    \caption{Quantitative results of each component. DWVSS is our Dynamic Weighted Video Sampling Strategy.}
    \label{tab:abalation}
\end{table}

==> tables/user_study.tex <==
% \begin{table}[]
%     \small
%     \centering
%     \resizebox{0.48\textwidth}{!}{
%     \begin{tabular}{ccccc}
%     \toprule
%     Method           & Subject Fidelity & Motion Fluency & Text Alignment & Overall Quality \\ \midrule
%     Custom Diffusion & 28.24\%          & 9.56\%          & 9.70\%           & 14.18\%            \\
%     DreamVideo       & 27.48\%          & 19.85\%         & 14.93\%          & 11.19\%            \\
%     Ours             & 44.28\%          & 70.59\%         & 75.37\%          & 74.63\%           \\ \bottomrule
%     \end{tabular}}
%     \captionsetup{font={small}}
%     \caption{User Study.}
%     \vspace{-1.0cm}
%     \label{tab:user}
% \end{table}

\begin{table}[]
    \small
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{ccccc}
    \toprule
    Method           & Subject Fidelity & Motion Fluency & Text Alignment & Overall Quality \\ \midrule
    Custom Diffusion & 25.82\%          & 17.15\%         & 12.74\%          & 14.57\%            \\
    DreamVideo       & 21.66\%          & 22.16\%         & 14.69\%          & 11.70\%            \\
    \textbf{Ours}             & \textbf{52.52\%}          & \textbf{60.69\%}         & \textbf{72.57\%}          & \textbf{73.73\%}           \\ \bottomrule
    \end{tabular}}
    \captionsetup{font={small}}
    \caption{The result of a user study with 20 participants.}
    \label{tab:user}    
\end{table}
